End-to-end optimized image compression for multiple machine tasks

An increasing share of captured images and videos are transmitted for storage and remote analysis by computer vision algorithms, rather than to be viewed by humans. Contrary to traditional standard codecs with engineered tools, neural network based codecs can be trained end-to-end to optimally compress images with respect to a target rate and any given differentiable performance metric. Although it is possible to train such compression tools to achieve better rate-accuracy performance for a particular computer vision task, it could be practical and relevant to re-use the compressed bit-stream for multiple machine tasks. For this purpose, we introduce 'Connectors' that are inserted between the decoder and the task algorithms to enable a direct transformation of the compressed content, which was previously optimized for a specific task, to multiple other machine tasks. We demonstrate the effectiveness of the proposed method by achieving significant rate-accuracy performance improvement for both image classification and object segmentation, using the same bit-stream, originally optimized for object detection.

==> 01_abstract.tex <==
\begin{abstract}

An increasing share of captured images and videos are transmitted for storage
and remote analysis by computer vision algorithms, rather than to be viewed by humans.
Currently deployed image/video codecs feature engineered tools that are challenging to
optimize for such machine task algorithms. However, neural network based codecs can be trained
end-to-end to optimally compress images with respect to a target rate and any
given differentiable performance metric. In this paper, we
consider such optimized end-to-end compression and task
framework, consisting of a differentiable codec and different task algorithms
that are applied to the decoded images.
Although it is possible to train compression tools to achieve better
rate-accuracy performance for a particular computer vision task, it could be practical and relevant
to re-use a compressed bit-stream for multiple machine tasks. For this purpose, we introduce connectors that are inserted between the decoder and the task algorithms to enable a direct
adaptation of the compressed content, which was previously optimized for a
specific task, to multiple other machine tasks. We demonstrate the
effectiveness of the proposed method by achieving significant rate-accuracy
performance improvement for both image classification and object segmentation,
using the same bit-stream, originally optimized for object detection.

\end{abstract}



==> 02_introduction.tex <==
\section{Introduction}


\begin{figure}[t]
	\setlength{\tabcolsep}{1pt}
	\footnotesize
	\centering
	\begin{tabular}{llll}
		Rate-Distortion & Rate-Detection& Rate-Distortion&Rate-Multi task\\
		\includegraphics[width=0.234\linewidth]{figures/sameBPP/bearQ1HP.png}&
		\includegraphics[width=0.234\linewidth]{figures/sameBPP/bearQ2Joint.png}&
		\includegraphics[width=0.255\linewidth]{figures/imagenet/snowLQ1HP.png}&\hspace{-1mm}
		\includegraphics[width=0.255\linewidth]{figures/imagenet/snowLQ4JointConv.png}\\
		Acc mAP\@: 32.6 &34.1 (\textcolor{ForestGreen}{$+$}\textbf{4.6}\%)&Acc top-5: 66.43\%&75.18\% (\textcolor{ForestGreen}{$+$}\textbf{8.75}\%)\\
		%top-5:&&&top-5\%:\hspace{2mm}66.43&73.21 (\textbf{6.78}$\uparrow$)
		%&75.18\% (\textbf{8.75}$\uparrow$)\\
		PSNR\@: 30.49 dB &16.31 dB &26.37 dB &22.35 dB (\textcolor{red}{$-$}\textbf{4.02})
	\end{tabular}
	\vspace{1mm} % to make the figure clear
	\caption{End-to-end optimization of an ANN-based
		codec for multiple machine tasks. Left:
		the detection accuracy is improved by 4.6\% at the same bitrate by
		optimizing the codec from~\cite{balle2018variational} for rate-detection instead of the
		conventional rate-distortion based on PSNR (`bear' image from
		COCO~\cite{lin2014microsoft}). Right: We show that it is possible to use
		a rate-`object detection' optimized codec to achieve high rate-`multi
		task accuracy' performances (classification, segmentation, etc.),
		 using the proposed simple pre-trained connectors. `Tiger' from
		ImageNet-1K~\cite{russakovsky2015imagenet} is compressed using the same
	rate-`object detection' optimized codec coupled with a trained connector (81
parameters) to achieve a 8.75\% image classification accuracy improvement on an
off-the-shelf classifier (right image).}
\label{fig:main}
\end{figure}

The development of efficient Graphics Processing Units (GPUs), the increasing
use of IoT (Internet of Things) devices and the success of deep learning
algorithms in solving data driven problems have given rise to a myriad of use
cases and requirements in terms of machine-to-machine image and video transmission.
 %   For instance, Augmented and Virtual Reality (AR-VR) mobile traffic is
%   expected to grow 12 times in 2022 compared to 2017~\cite{forecast2019cisco}.
Many computer vision tasks, such as object detection, tracking, image
classification, etc., rely on computationally challenging algorithms that cannot be
run on embedded devices, and require the content to be transmitted to remote
servers. Hence the emerging research field of `Video Coding for Machines'
(VCM) aims to develop optimized compression methods for video content that is
meant to be analyzed by machines, rather than viewed by human
users~\cite{duan_video_2020}.

Existing compression standards rely on handcrafted hybrid architectures that aim
to remove the redundancies in the source signal and often require further
compression using quantization, introducing image distortion. Traditional image
and video standards, such as JPEG~\cite{jpeg}, H.264/AVC~\cite{avc},
H.265/HEVC~\cite{hevc} and AV1~\cite{av1}, are designed to minimize the
distortion in terms of visual quality. Hence these codecs are optimized for
`rate-distortion' and are not necessarily optimal for other machine tasks such
as object detection, classification, or segmentation.

Contrary to conventional hybrid compression frameworks, Artificial Neural
Networks (ANN)-based codecs can be directly optimized with respect to any loss
function measuring performance, not limited to traditional signal fidelity such as
Peak Signal-to-Noise Ratio (PSNR)\@. In particular, when machine task architectures are known, a
prediction loss based on the algorithm's accuracy on decoded images can be used
to optimize the parameters of the codec as well. It is then possible to jointly
optimize the end-to-end system consisting of the codec and the task algorithm,
considering a rate-`task accuracy' criterion instead of rate-distortion.
Fig.~\ref{fig:main} depicts this trade-off between the distortion and object
detection metrics. Optimizing the codec on a `rate-distortion' criterion leads
to a better image visual quality whereas optimizing on rate-detection results in
a higher accuracy and a poorer visual quality (but still viewable).

As illustrated in Fig.~\ref{fig:main}, one major drawback of end-to-end optimization of a codec for a specific task is the distortion in visual quality of the reconstructed images. This obstructs the use of such images on available off-the-shelf task models (designed for different applications) trained with rate-distortion optimized inputs resulting poor inference performance. Hence there is a clear design trade-off between the rate-accuracy performance of an end-to-end optimized bit-stream for a desired primary task and secondary machine tasks including viewing. Therefore a study of compressing source images/videos to features that are generic enough to be used for multiple machine tasks at the receiver is of practical importance. For example, a system might be optimized for
object detection or classification for video surveillance, but
visualization may also be required later if the videos are used as
pieces of evidence. 

% Following the current trends in hardware improvement, sensors can now be coupled with GPUs which enables learning features from image/video content at compression, while optimizing to analyze for multiple machine tasks.
%	
As the main contribution of the this paper, following an in-depth study of a framework consisting of a trainable auto-encoder based codec and machine task algorithms that are applied to the
decoded frames, we introduce post-decoding connectors to adapt the decoded content to different secondary tasks, and retrieve most of the accuracy loss due to
compression artifacts. The proposed connectors enable to `de-specialize'
the decoded images, producing a content that is more generic to be
used for secondary purposes.

The remainder of the paper is organized as follows. Related work is first
discussed in Sec.~\ref{sec:related}. In Sec.~\ref{sec:study}, a study is
provided with extensive experimental results of different configurations for the
optimization of machine task accuracy under bit-rate constraints. %, including the
%fine-tuning of the different parts of the chain.
 Then, the proposed connectors
are described in Sec.~\ref{sec:reuse} to enable the use of the jointly
fine-tuned codec for secondary tasks. Finally the conclusions are discussed in Sec.~\ref{sec:conclusion}.
Additional visual examples and details of the experiments are given in the
supplemental material.


==> 03_related_work.tex <==
\section{Related works}
\label{sec:related}

	Numerous ANN-based auto-encoders have been proposed in recent years, which now outperform some of the conventional standard codecs such as JPEG~\cite{jpeg}, JPEG2000~\cite{jpeg2k}, H.264/AVC~\cite{avc} and H.265/HEVC~\cite{hevc} in terms of rate-distortion performance.

	The auto-encoder models presented in \cite{toderici2017full} consists of LSTM units with convolutions for image compression in order to capture the conditional relationship among neighboring pixels.
	The authors of \cite{balle2018variational} proposed an auto-encoder transforming the input image into a tensor or latent, which is encoded using another auto-encoder which generates side information called `hyperpriors' to estimate the distribution of latent representation.
	We will refer to this model as \textit{bmshj2018-hyperprior} in the remainder of this paper.
	For image compression, the work \cite{mentzer2018conditional} utilized a model with both the encoder and decoder designed with residual blocks and skip connections.
	Similarly the authors of \cite{habibian2019video} utilized variational auto encoder concepts for video compression.  %These auto-encoders mainly rely on building blocks of convolutional layers and generalized divisive normalization (GDN) joint non-linearities that have proven effective for modeling the image space.
	All the above works~\cite{balle2018variational,habibian2019video,mentzer2018conditional, toderici2017full} used a trainable context model for probability estimation and established that it is essential to learn the code-word distribution for efficient compression instead of using fixed code-word tables as in JPEG and JPEG2000.

	In terms of optimizing image/video compression codecs for a given learning task, only a handful of works emerges from the literature.
	The authors of \cite{luo2020rate} and \cite{chamain2018QuanNet} proposed to learn the quantization tables of JPEG and JPEG2000, respectively, using end-to-end training for image classification with differential codec implementations.
	The method presented in \cite{luo2020rate} shows performance gain in `rate-distortion-accuracy' by training a differentiable implementation of JPEG codec with a MobileNet fixed classifier~\cite{howard2019searching}.
	They discussed how the learned features generalize over different architectures for the same learning task by observing that the codec learned for the MobileNet~\cite{howard2017mobilenets} classifier achieves similar gains with a ResNet~\cite{he2016deep} classifier.
	The rate-accuracy performance of both works \cite{luo2020rate, chamain2018QuanNet} is likely sub-optimal since the JPEG and JPEG2000 have a pipeline consisting of human engineered blocks for visual quality, limiting the degree of freedom to fully optimize  the codec for a given machine task other than visualization. 

	In contrast to \cite{luo2020rate}, our work focuses on optimizing the codec and task model for rate-accuracy performance, without considering the image quality in the training loss function. Unlike in \cite{chamain2018QuanNet}, our approach has the advantage of enabling the use of off-the-shelf task models on the decoded images.
	To the best of our knowledge, this is the first work that discusses how to reuse the feature maps optimized for one task on multiple other learning tasks, including viewing.
	In particular, we take a step further from \cite{luo2020rate} and show that the end-to-end optimized features are valid for multiple tasks. % as well showing significant performance gains. %In contast to us, they maintain the similar image quality (PSNR) hence the gains are marginal. We show simialr ImageNet-1K accuracy improvement with the codecs optimized for a different task and a dataset. Further the classification gain reducess with higher BPP like ours.
	%{\color{red}End-to-end optimization for p frame compression. \cite{wu2020end}}.

==> 04_machine_task.tex <==
\section{On end-to-end optimized compression for machine task}\label{sec:study}%

\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/codec_task4.png}
	\caption{General structure of networked ML use case: input $\mathbf{x}$ is encoded to latent $\mathbf{z}$ and stored/transmitted over a channel as a binary stream. The decoder decodes the binary stream and reconstructs $\mathbf{\hat x}_q$ on which the the learning/inference is performed by the task model.}\label{fig:structure}
\end{figure}

% \subsection{Structure of networked codec and task algorithm}
The considered networked Machine Learning (ML) inference applications observe the general structure shown in Fig.~\ref{fig:structure}. It consists of a `codec' that efficiently compresses the input $\mathbf{x}$ which can be reconstructed at quality `$q$' ($\mathbf{\hat x}_q$)  and a `task model' that performs the learning task $T$ on the reconstructed image $\mathbf{\hat x}_q$. We parameterize the codec that encodes images at quality $q$ with $\boldsymbol \psi_q$, ($\mathbf{\hat x}_q = \boldsymbol \psi_q(\mathbf{x})$) and the task model with $\boldsymbol \theta$.

In general, the codec consists of an Encoder Analyzer (E), an Entropy Coder (EC), an Entropy Decoder (ED) and a Decoder Synthesizer (D). The Encoder Analyzer transforms the input image $\mathbf{x}$ into a lower dimensional, quantized latent representation $\mathbf{z}$ which is compressible. The Entropy Coder estimates the probabilities of the elements of $\mathbf{z}$ and generates a binary stream of entropy $H(\mathbf{z})$ which is stored or transmitted over a potentially low bandwidth wireless channel. The Entropy Decoder decodes the bit stream to reproduce $\mathbf{z}$ and the Decoder synthesis stage reconstructs $\mathbf{\hat x}_q$ from $\mathbf{z}$.
During inference, a pre-trained task model $\boldsymbol \theta$ performs the learning on $\mathbf{\hat x}_q$ and estimates the result $y$, ($\boldsymbol \theta(\mathbf{\hat x}_q)=y$). For instance, in image classification $y$ is the estimated class label. The inference accuracy can be calculated by considering the difference between the estimated label $y$ and the ground truth label $y_{gt}$ for $\mathbf{x}$ given the availability. In general, the task model $\boldsymbol \theta$ is optimized for minimum task loss on the input images of best possible (reference) quality `$rq$' available during training. We denote the task model optimized for the reference quality $rq$ by $\boldsymbol \theta_{rq}$.

\subsection{Task specific optimization}
We explore 4 main settings related to training the codec and the task model. As the first setting, we explore the rate-accuracy performance for a selected primary task $T$ by performing the inference on off-the-shelf (baseline) model $\boldsymbol \theta_p$ with the inputs generated by a rate-distortion optimized codec $\boldsymbol \psi_q$. In the second setting we fine-tune the task model (T-FT) for the rate-distortion optimized codec. Third setting explores the rate-accuracy performance by fine-tuning the codec (C-FT) for an off-the-shelf task model. As the final setting we jointly end-to-end optimize the codec and the task model (J-FT) for rate-accuracy performance of task $T$.

\subsubsection{Inference on off-the-shelf task model: baseline}
\label{sec:baseline}
 In this study, the source images are considered to be at the reference quality $rq$ on which almost all the deep learning (off-the-shelf) models are designed and optimized to perform tasks such as object detection, segmentation, tracking. By performing inference on these images that we further compress at different quality ratio $q$, ($\mathbf{\hat x}_q$), we can observe the performance in terms of rate vs. task accuracy (rate-accuracy) for each chain, codec followed by the  task model as shown in Fig.~\ref{fig:structure}. This forms the baseline for the proposed methods in this paper, referred to as `baseline' in the remainder of the paper.

%etc. have been trained on compressed images or frames of videos at the best available quality $rq$. (sometimes on raw images/videos).
%Under this setting, we perform object detection on COCO dataset with off-the-shelf pre-trained Faster-RCNN model ($\boldsymbol \theta_p$) as the detector and use VVC~\cite{chen_jvet-q2002_2020} and Scale hyperpriors~\cite{balle2018variational} as codecs for image compression.

\subsubsection{Fine tuning the task model only: T-FT}
\label{sec:T-FT}
Assume that $\mathcal{X}_{rq}$  denotes the set containing reference quality images $\mathbf{x}\in\mathcal{X}_{rq}$ and  $\mathcal{\hat X}_q$ denotes the set of images compressed and decompressed at a given quality $q$ as $\mathbf{\hat x}_q\in\mathcal{\hat X}_q$. $y_{gt}^{T} \in \mathcal{Y}^{T}$ is the ground truth for the inputs $\mathbf{x}$ and $\mathbf{\hat x}_q$ for the considered task $T$. Note that 
since mostly available codecs $\boldsymbol \psi^{D}_q$ are optimized for Distortion ($D$), we omit the superscript $D$ for notational simplicity and write $\mathbf{\hat x}_q =    \boldsymbol \psi_q(\mathbf{x})$. We express the loss function for a task $T$ with $\mathcal{L}_T(\boldsymbol \theta(\mathbf{\hat x}_q),y_{gt}^{T})$ which calculates task loss based on the prediction $y$ generated by the task model $\boldsymbol \theta$ for the input and the ground truth pair $(\mathbf{\hat x}_q,y_{gt}^{T})$ for task $T$.

Given that we have the access to the task model training and inputs (images) compressed at each quality ratios $q$, we can train the task model $\boldsymbol{\theta}$ with the images, $\mathbf{\hat{x}}_q$ to obtain a fine tuned task model $\boldsymbol \theta_q$ as given in Eq.~\eqref{eq:V2}. This leads to performance gain in task accuracy for a given rate.
\begin{align}
	\label{eq:V2}
	\boldsymbol \theta_q = \arg \min_{\boldsymbol \theta|\boldsymbol \theta_{rq}}  \dfrac{1}{|\mathcal{\hat X}_q|}\sum_{\mathbf{\hat x}_q ,y_{gt}^{T} \in\mathcal{\hat X}_q, \mathcal{Y}^{T}} \mathcal{L}_T(\boldsymbol \theta(\mathbf{\hat{x}}_q),y_{gt}^{T})
\end{align}
Note that search for optimal $\boldsymbol \theta$ is initialized with the off-the-shelf $\boldsymbol \theta_{rq}$ denoted by $\boldsymbol \theta|\boldsymbol \theta_{rq}$.

\begin{comment}
To validate the study, we chose to start with a well studied task on a well-known dataset. We selected object detection with COCO-2017 as the main task $T$ to be end-to-end optimized. After the end-to-end optimization, we use the learned Scale hyperprior codec $\psi_\beta^J$ as the codec that generates the rate-accuracy$_T$ optimized images. Hence these images ${\hat x}_\beta^J$ are generated from the rate-accuracy$_T$ optimized latents/feature maps. Then we used image classification on ImageNet-1K $S_1$ and pixel level video semantic segmentaion on Cityscapes $S_2$ as secondary tasks that use ${\hat x}_\beta^J$ as the input for inference anf fine tuning. We show that the images that are rate-accuracy$_T$ optimized can outperform the existing (can we use state-of-art?) rate-accuracy$_{S_1}$ and rate-accuracy$_{S_2}$ performance in both inference and fine-tuning.
\end{comment}
\subsubsection{Fine tuning the codec only: C-FT}
\label{sec:expV3}
Under the assumption that the graph of task model is known and the task loss can be back-propagated through the task model, we can fine tune the codec $\boldsymbol \psi$ by optimizing the parameters of the codec $\boldsymbol{\psi}$ without updating the task model $\boldsymbol \theta$. We minimize the the following loss to obtain a codec $\boldsymbol \psi_{\beta}^T$ s.t.,
\begin{align}
	\label{eq:V3}
	\boldsymbol \psi_{\beta}^T = \arg \min_{\boldsymbol \psi|\boldsymbol \psi_q} \dfrac{1}{|\mathcal{X}_{rq}|} \sum_{\mathbf{x} ,y_{gt}^{T} \in\mathcal{ X}_{rq}, \mathcal{Y}^{T}} &  \{\mathcal{L}_T(\boldsymbol \theta_{rq}(\boldsymbol \psi(\mathbf{x})),y_{gt}^{T}) \nonumber\\ & + \beta \mathcal{L}_R(\mathbf{z})\}
\end{align}

$\mathcal{L}_R(\mathbf{z})$ denotes the bandwidth/rate of the latent representation $\mathbf{z}$, which is the output of the encoder E of the codec $\boldsymbol{\psi}$ s.t. $\mathbf{z} = \rm E_{\boldsymbol{\psi}}(\mathbf{ x})$ as given in Fig.~\ref{fig:structure} during transmission. The control parameter $\beta$ regulates the trade-off between the task $T$ accuracy and the bandwidth/rate of the input to the task model.
\subsubsection{Joint end-to-end fine tuning: J-FT}
When we have access to training of both the codec and the task model we can choose to jointly optimize the parameters $\boldsymbol \psi$ and $\boldsymbol \theta$ to converge at better rate-task accuracy performance. Hence, We can find the optimal codec-task model combination ($\boldsymbol \psi_{\beta}^J,\boldsymbol \theta_{\beta}^J$) as follows.
\begin{align}
	\label{eq:V4}
	\boldsymbol \psi_{\beta}^J&, \boldsymbol \theta_{\beta}^J \nonumber\\&= \arg \min_{\boldsymbol \psi|\boldsymbol \psi_q,\boldsymbol \theta|\boldsymbol \theta_{rq}} \dfrac{1}{|\mathcal{ X}_{rq}|} \sum_{\mathbf{x} ,y_{gt}^{T} \in\mathcal{ X}_{rq}, \mathcal{Y}^{T}} \{\mathcal{L}_T(\boldsymbol \theta(\boldsymbol \psi(\mathbf{x})),y_{gt})\nonumber\\ &\qquad\qquad\qquad\qquad\qquad\qquad\qquad\quad+ \beta \mathcal{L}_R(\mathbf{z})\}
\end{align}

We initialize the codec and the task model with off-the-shelf pre-trained models $\boldsymbol \psi_q$ and $\boldsymbol \theta_{rq}$ for each $\beta$ value at the beginning of the training.
%{\color{red} Decoder fixed training, what's the reason behind this?-no need to write equations.}
\subsection{Experiments and Results}
In this section we provide the details of the experiment setup and results. To test the previously described settings, we used the well researched object detection on COCO-2017~\cite{lin2014microsoft} data set as task $T$.
COCO-2017 dataset for object detection contains over 180k training and 5k validation RGB images of average size over 256$\times$256 with annotated bounding boxes belonging to 80 classes. We used the standard primary challenge metric `box mAP' at 10 Intersection over Union (IoU) values between 0.50 and 0.95\footnote{\url{https://cocodataset.org/\#detection-eval}}
to evaluate the detection accuracy of the val set. As the detection model on the COCO-2017 data set, we used Faster-RCNN~\cite{ren2015faster} with ResNet-50 backbone throughout the experiments.

As the baseline image codecs for the current work, we used  VVC~\cite{chen_jvet-q2002_2020} and Scale hyperpriors model \textit{bmshj2018-hyperprior}, optimized on MSE~\cite{balle2018variational}. VVC is the current state-of-art video standard which can also be used for still image compression. For VVC, we used the reference software VTM-8.2 in still picture mode to compress the images during this study (See the supplemental material for more details). \textit{bmshj2018-hyperprior} is an auto encoder-decoder based differentiable codec featuring an entropy coder that efficiently compress prior information achieving better rate-distortion performance compared to ANN based codecs proposed in ~\cite{johnston2018improved,toderici2017full}.
\subsection{Inference and Fine tuning the task model: \quad baseline, T-FT}
\label{sec:exp:V2}
For the inference (baseline), we used off-the-shelf pre-trained Faster-RCNN detector which is available \href{https://github.com/open-mmlab/mmdetection}{online}~\cite{mmdetection}.
In order to obtain a rate-accuracy point for VVC codec, we set the quality parameter $QP$ of the VVC encoder at a certain value and generated the bit-stream for each image.
Then we reconstructed the RGB images at the VVC decoder using the produced bit-stream and stored the images to use as the input for the off-the-shelf detector to calculate the accuracy during inference. The size of the bit-stream was used to calculate the rate in bits per pixel (BPP) for each image. We generated the rate-accuracy curve by repeating this process for $QP\in\{47,42,37,32,27,22,17\}$. Smaller $QP$ generates better quality images.

\begin{figure}[t]
	\centering
	\includegraphics[trim=10 10 40 20,clip,width=1.0\linewidth]{figures/cocoV1V2old_3.pdf}
	\caption{rate-accuracy comparison for VVC and Scale hyperpriors. Solid-setting baseline: inference. Dash-setting T-FT: fine tuning the task model}\label{fig:baselineCOCOold}
\end{figure}

For \textit{bmshj2018-hyperprior} codec, we used the off-the-shelf pre-trained models optimized for MSE, available at~\cite{CompressAI}. Similar to VVC, we changed the quality parameter $q\in [1,8]$ of \textit{bmshj2018-hyperprior} codec and generated images at different BPP for inference. To observe the performance gain for T-FT setting as given in Eq.~\eqref{eq:V2}, we fine tuned the Faster-RCNN model starting from the off-the-shelf pre-trained parameters with a stochastic gradient optimizer at a learning rate of $0.01$ for 6 epochs. For each rate-accuracy point for both VVC and \textit{bmshj2018-hyperprior}, we used the images compressed at each BPP separately during fine-tunning the detector.

Fig.~\ref{fig:baselineCOCOold} compares the performance in terms of detection accuracy vs. bitrate between the baselines for inference (baseline) and T-FT setting. Fine-tuning the task algorithm on reconstructed images unsurprisingly improves rate- accuracy trade-offs, especially at low bit-rates. Interestingly, in both cases the two codecs perform similarly in terms of rate-accuracy, while the \textit{bmshj2018-hyperprior} cannot compete against VVC in PSNR~\cite{CompressAI}.

\subsection{Fine tuning the codec only: C-FT}
\label{sec:exp:V3}
We fine tuned the  \textit{bmshj2018-hyperprior} codec with a fixed off-the-shelf pre-trained detector to minimize the loss given in Eq.~\eqref{eq:V3}.
To obtain a rate-accuracy point during fine-tuning, we initialized the codec with pre-trained parameters optimized for MSE at given quality $q$ and selected the control parameter $\beta$ accordingly.
Table~\ref{tab:V3}  lists the $\beta$ values we used to achieve each rate and quality of scale hyperprior model used for parameter initialization.
\begin{table}[t]
	\centering
	\begin{tabular}{lcccc}
		\toprule
		Initial codec quality ($q$) &1&2&4&4\\	\midrule
		Control parameter ($\beta$) &1.0&0.6675&0.3186&0.1\\
		\bottomrule
	\end{tabular}
	\vspace{1mm} % to make the figure clear
	\caption{Hyper-parameter settings for C-FT and J-FT. We initialize the codec with pre-trained weights for quality $q$ at each $\beta$ value.}\label{tab:V3}
\end{table}
We fine-tuned the codec for 6 epochs on COCO-2017 training set with an Adam optimizer with a batch size of 2 at a learning rate of $10^{-4}$.

Fig.~\ref{fig:cocov4_DF} compares the results of the proposed settings. Note that retraining the codec only (C-FT) under-performs task fine-tuning (T-FT), but still
improves significantly over the off-the-shelf codec.

\begin{comment}
\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.7\linewidth]{figures/cocoV3.png}
\end{center}
\caption{Fine tuning the image codec for a fixed task model}
\label{fig:cocov3}
\end{figure}
\end{comment}


\subsection{Joint end-to-end fine tuning: J-FT}
For joint end-to-end optimization of both the codec and the detector following Eq.~\eqref{eq:V4}, we fine tuned the codec and the detector for 5 epochs with the same optimizers and learning rates we used in C-FT and T-FT in Sec.~\ref{sec:exp:V3} and \ref{sec:exp:V2} respectively using the parameter settings in Table~\ref{tab:V3}.
Since \textit{bmshj2018-hyperprior} codec training is an easier learning task compared to the detection with Faster-RCNN model, we fine tuned the detector for 1 additional epoch (6 epochs in total) with the codec fixed at epoch 5.
We observed that this strategy gains over 7.1\% and 1.6\% detection accuracy improvement at 0.08bpp and 0.25bpp respectively over concurrent training of the codec and the detector for 6 epochs. Note that in Fig.~\ref{fig:cocov4_DF}, J-FT outperforms all the other other settings in rate-accuracy performance significantly at lower bit rates.

With the purpose of having a universal decoder on different target devices, we fixed the decoder of \textit{bmshj2018-hyperprior} codec and repeated the end-to-end training without updating decoder parameters to generate the rate-accuracy performance curves denoted as J-FT-FD. Interestingly for J-FT-FD, the performance drop is significantly small compared to J-FT. See Fig.~\ref{fig:cocov4_DF}. 
\begin{comment}
\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.7\linewidth]{figures/cocoV4.png}
\end{center}
\caption{End-to-end training performance comparison}
\label{fig:cocov4}
\end{figure}
\end{comment}
\begin{figure}[t]
	\centering
	\includegraphics[trim=10 10 40 20,clip,width=1.0\linewidth]{figures/cocoV4FD_4.pdf}
	\caption{Rate-accuracy performance for object detection on COCO-2017 val set with scale hyper-prior image codec.
		Original: detection accuracy on raw images, baseline: inference on off-the self codec+detector.
		T-FT: fine tuning the detector, C-FT: fine-tuning the codec for rate-accuracy.
		J-FT: end-to-end fine tuning the codec and the detector for rate accuracy. J-FT-FD: J-FT with fixed decoder.}\label{fig:cocov4_DF}
\end{figure}

\subsection{Comparing visual quality of the end-to-end optimized images}
 Since the loss functions in Eq.~\eqref{eq:V3} and \eqref{eq:V4} do not contain a distortion term on the reconstructed images, the above described settings C-FT and J-FT are not optimized for viewing. In Fig.~\ref{fig:reconCompare1}  we compare the visual quality of the reconstructed RGB image of the image `bear' from COCO-2017 validation data set that achieves similar detection accuracy for the proposed settings.
\begin{figure}[t]
	\footnotesize
	\setlength{\tabcolsep}{1pt}
	\centering
	\begin{tabular}{llll}
		%\toprule
		Original & T-FT&C-FT &J-FT\\	%\midrule
		\includegraphics[width=0.24\linewidth]{figures/sameAP/original.jpg}&
		\includegraphics[width=0.24\linewidth]{figures/sameAP/bearQ2HP.png}&
		\includegraphics[width=0.24\linewidth]{figures/sameAP/bearQ4Enc.png}&
		\includegraphics[width=0.24\linewidth]{figures/sameAP/bearQ2Joint.png}\\
		%\midrule
		box mAP&34.4&34.2&34.1\\
		PSNR (dB)&32.11&20.01&16.31\\
		BPP&0.1461(\textcolor{ForestGreen}{$+$}\textbf{54.9\%})&0.1736(\textcolor{ForestGreen}{$+$}$ \textbf{84.1}\%$)&0.0943\\
	\end{tabular}
	\vspace{1mm} % to make the figure clear
	\caption{Reconstructed images from the latent space with detection accuracy 34-34.5 box mAP. The settings T-FT and C-FT demands over $50\%$ rate for the same detection accuracy compared to the proposed J-FT setting. }\label{fig:reconCompare1}
\end{figure}
End-to-end optimization achieves over $50\%$ bandwidth savings compared to using distortion (MSE) optimized scale hyper-priors for detection accuracy in the range of 34-34.5 box mAP. 

Fig.~\ref{fig:reconCompare2} compares the visual quality of the reconstructed RGB 'bear' image with the similar rate. We observe over 4.5\% improvement of the detection accuracy with end-to-end training compared to fine tuning the detector (T-FT) at rate point 0.1bpp.
\begin{figure}[t]
	\footnotesize
	\setlength{\tabcolsep}{1pt}
	\centering
	\begin{tabular}{llll}
		%\toprule
		Original & T-FT&C-FT &J-FT\\	%\midrule
		\includegraphics[width=0.24\linewidth]{figures/sameBPP/original.jpg}&
		\includegraphics[width=0.24\linewidth]{figures/sameBPP/bearQ1HP.png}&
		\includegraphics[width=0.24\linewidth]{figures/sameBPP/bearQ1Enc.png}&
		\includegraphics[width=0.24\linewidth]{figures/sameBPP/bearQ2Joint.png}\\
		%\midrule
		box mAP&32.6&29.8&34.1 (\textcolor{ForestGreen}{$+$}\textbf{4.6}\%)\\
		PSNR (dB)&30.49&17.70&16.31\\
		BPP&0.1024&0.0827&0.0943
	\end{tabular}
	\vspace{1mm} % to make the figure clear
	\caption{Reconstructed images from the latent space with rate $\approx$ 0.1bpp. The proposed J-FT gains 4.6\% detection accuracy compared to T-FT setting.}\label{fig:reconCompare2}
\end{figure}
Note that the reconstructed images for the setting J-FT: end-to-end optimized for detection highlights features which help improving detection accuracy compared to the images optimized for visual distortion (T-FT).% These highlighted features can be seen as artifacts by the models trained with high quality images for other learning tasks such as image synthesis for viewing, segmentation etc.


==> 05_discussion.tex <==
\subsection{Effect of connectors on visualization}\label{sec:Discussion}%

\begin{figure}[t]
	\setlength{\tabcolsep}{1pt}
	\centering
	\footnotesize
	\begin{tabular}{rccc}
		%\toprule
		Original & J-FT&J-FT Avg pool& J-FT Conv\\	%\midrule
		\includegraphics[width=0.24\linewidth]{figures/imagenet/snowLOri.JPEG}&
		\includegraphics[width=0.24\linewidth]{figures/imagenet/snowLQ1Joint.png}&
		\includegraphics[width=0.24\linewidth]{figures/imagenet/snowLQ1JointAvpool.png}&
		\includegraphics[width=0.24\linewidth]{figures/imagenet/snowLQ1JointConv.png}
		\\
		%\midrule
		PSNR&16.24&18.42&19.83\\
		BPP&0.1119&0.1119&0.1119\\
		%\midrule
		&
		\includegraphics[width=0.24\linewidth]{figures/imagenet/snowLQ4Joint.png}&
		\includegraphics[width=0.24\linewidth]{figures/imagenet/snowLQ4JointAvpool.png}&
		\includegraphics[width=0.24\linewidth]{figures/imagenet/snowLQ4JointConv.png}
		\\
		%\midrule
		PSNR&19.94&21.90&22.35\\
		BPP&0.2203&0.2203&0.2203\\
		%\midrule
		%\bottomrule
	\end{tabular}
	\vspace{1mm}
	\caption{Comparison of the quality of the 'tiger' image from ImageNet-1K validation set. Columns J-FT: image generated by end-to-end optimized \textit{bmshj2018-hyperprior}, J-FT Avg pool: J-FT transformed by average pooling connector, JFT Conv: JFT transformed by the 2D conv. connector.}\label{fig:tiger}
\end{figure}


Contrary to the method described in~\cite{luo2020rate}, our loss function expressed in
Eq.~\eqref{eq:V4} does not include any criterion related to the visual quality
of decoded images, or distortion constraints with respect to the original
signal. Fig.~\ref{fig:tiger} shows the reconstructed images from the output of
average pooling (J-FT Avg pool) and 2D convolution filters (J-FT Conv). It is clear that the codec optimized
for object detection produces images that include high frequency features, which
help detecting objects. In the case of image classification as secondary task,
the connector learns to smoothen the decoded images from the rate-detection
optimized codec to match the color, brightness and patterns required for
classification. Once those details are captured by a simple connector,
re-training of the connector for different tasks and data sets is unnecessary.
In both cases, the original signal is heavily distorted, both visually and
quantitatively (PSNR), but the images are still viewable, which can be useful
for explain-ability. Further details on this, including PSNR and MS-SSIM curves on the COCO dataset, are provided in supplement. 

\section{Conclusion}\label{sec:conclusion}

In this paper, we provided an in-depth study of an end-to-end optimization of an image
compression codec for a primary learning task (object detection) under bit-rate constraints, including the fine-tuning of the different parts of the chain. The experiments demonstrate that
it is possible to significantly improve the task accuracy when fine-tuning
jointly the codec and the task network for object detection, especially at low
bit-rates.

To be able to re-use the content decoded from the compressed bit-stream originally optimized for object detection, for other secondary vision tasks, such as image
classification and segmentation, we introduced simple pre-trained connectors with a small number of
parameters (maximum 81 in the case of 2D convolution). Based on the experiments on ImageNet-1K and Cityscapes data sets, we showed that the proposed connectors achieve significantly better rate-accuracy performance compared to the conventional codecs optimized for rate-distortion. In the future work, we plan to explore the applicability of the connectors in video compression for multiple machine tasks.


==> 05_multi_tasks.tex <==
\section{Re-usability of decoded pictures for multi-task use cases}
\label{sec:reuse}%

%\subsection{Can we use the decoded frames for another task?}
In this section, we explore the re-usability of the latent/feature maps generated from the end-to-end optimized codec $\boldsymbol \psi_{\beta}^J$ for task $T$ during training and inference on a secondary task $S$ parameterized by $\boldsymbol \phi$. We observe on Figures~\ref{fig:reconCompare1} and \ref{fig:reconCompare2} that images generated by the jointly optimized codec $\boldsymbol \psi_{\beta}^J$ show highlighted feature patterns, compared to the images generated by the codecs optimized for MSE-based rate-distortion $\boldsymbol \psi_q^D$. These patterns can be seen as artifacts by the models trained with high quality images for other learning tasks such as image synthesis for viewing, segmentation etc.%These patters can be called artifacts when used for visualization purposes.

\subsection{Introducing Connectors}
\label{sec:reuse-connectors}
Due to the presence of these artifacts, the end-to-end optimized inputs $\mathbf{\hat x}_\beta^J$ perform poorly in terms of rate-accuracy performance for task $S$ on a pre-trained off-the-shelf task model $\boldsymbol \phi_{rq}$ trained with rate-distortion optimized inputs. So it's essential to de-specialize the jointly optimized inputs before using them for secondary tasks. For this purpose, we add a Connector $C$ parameterized by $\boldsymbol c$ in between the codec output $\mathbf{\hat x}_\beta^J$ and the task model $\boldsymbol \phi_{rq}$. See Fig.~\ref{fig:featureReuse}. The goal of $C$ is to transform $\mathbf{\hat x}_\beta^J$ to $\mathbf{\hat x}^C_\beta$ which is the input to the model $\boldsymbol \phi_{rq}$.
\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/featureReuse3.png}
	\caption{Proposed feature reuse flow: The images generated by codec $\boldsymbol \psi_{\beta}^J$ optimized for the primary task, are transformed by a simple pre-trained connector $C$ before being used by the the off-the-shelf secondary tasks $S$ for inference.}\label{fig:featureReuse}
\end{figure}

With the proposed connector, the inference for secondary task  $S$ can be performed according to the following flow for the input, ground truth pair ($\mathbf{x}$, $y_{gt}^{S}\in \mathcal{Y}^{S}$). Here $y$ is the estimated label for task $S$.
 \begin{equation}
	\mathbf{x} \xrightarrow[\boldsymbol \psi_\beta^J]{\text{E-EC-ED-D}} \mathbf{\hat x}_\beta^J\xrightarrow[\boldsymbol c_{\beta}^{J}]{C} \mathbf{\hat x}^C_\beta\xrightarrow[\boldsymbol \phi_{rq}]{S}y
\end{equation}

In the context of re-usability of features that are originally optimized for a primary task, on off-the-shelf secondary task models, the codec $\boldsymbol \psi_\beta^J$ and the pre-trained model $\boldsymbol{\phi}_{rq}$ are fixed, hence beyond out control. We explore the possibility of a simple fixed/trainable connector that can be stored at the end devices that perform inference for multiple tasks. 

For trainable $C$ we propose to find the optimal parameter setting $\boldsymbol c_{\beta}^{J}$ that minimizes the distortion $\mathcal{L}_D$ between the connector produced image $\mathbf{\hat x}_\beta^C$ and its rate-distortion optimized version $\mathbf{\hat x}_q^D$. Therefore we find $\boldsymbol c_{\beta}^{J}$ s.t.
\begin{align}
	\label{eq:V5}
	\boldsymbol c_{\beta}^{J} = \arg \min_{\boldsymbol c}  \dfrac{1}{|\mathcal{X}_{rq}|}\sum_{\mathbf{ x}, \mathbf{\hat x}_q \in \mathcal{X}_{rq}, \mathcal{\hat X}_q}  \mathcal{L}_D(\boldsymbol c(\boldsymbol \psi_{\beta}^J(\mathbf{x})),\mathbf{\hat x}_q).
\end{align}

For each rate-accuracy control parameter $\beta$, the trained connector $\boldsymbol c_{\beta}^{J}$ can be stored at the decoder and used for images that were compressed with the codec $\boldsymbol \psi_\beta^J$ during inference of any secondary task. Note that the proposed optimization of $\boldsymbol c$ is independent of the secondary task $S$. Therefor training of the connector given in Eq.~\eqref{eq:V5} is only performed once and zero knowledge of the secondary task is required.
\subsection{Fine-tuning the task model with end-to-end optimized images: J-FT T-FT}
Given that we have the access to the secondary task model and training set, for better accuracy at task $S$, we can fine tune the task model $\boldsymbol \phi$ on images compressed and reconstructed using the end-to-end jointly optimized coded $\boldsymbol \psi_\beta^J$.

The fine-tuned task model $\boldsymbol \phi_{\beta}$ is obtained by minimizing the task loss $\mathcal{L}_S$ as the following at each rate specified by $\beta$.
\begin{align}
	\boldsymbol \phi_{\beta} = \arg \min_{\boldsymbol \phi|\boldsymbol \phi_{rq}}  \dfrac{1}{|\mathcal{X}_{rq}|}\sum_{\mathbf{ x} ,y_{gt}^{S} \in\mathcal{ X}_{rq}, \mathcal{Y}^S} \mathcal{L}_S(\boldsymbol \phi(\boldsymbol \psi_{\beta}^J(\mathbf{x})),y_{gt}^{S})
\end{align}
We initialize the task model $\boldsymbol \phi$ with off-the-shelf pre-trained model $\boldsymbol \phi_{rq}$ for each $\beta$ value at the beginning of the training.
\subsection{Experiments and Results}
In order to show that the latent/feature maps generated by the codec $\boldsymbol \psi_{\beta}^J$ optimized for the object detection task are reusable, we performed inference for image classification on ImageNet-1k~\cite{russakovsky2015imagenet}  and semantic segmentation on Cityscapes~\cite{cordts2016cityscapes}. ImageNet-1K consists of RGB images of size over 256$\times$256 belonging to 1000 classes, each class containing about 1300 training and 50 validation samples. We evaluated the performance of the classification task $S_1$ with the metrics top-1 and top-5 accuracy.

Cityscapes is a video dataset recorded in streets from 50 cities captured in 5000 frames split into 2975 training, 500 val and 1525 test sets. For our experiments we used the left frames of training and val set with fine annotations belonging to 19 classes. The task of per-pixel semantic labeling $S_2$ is to label each pixel into one of 19 classes measured by the metric IoU~\cite{cordts2016cityscapes}.

Fig.~\ref{fig:imagenetCOCO}(a) shows the top-1 accuracy for ImageNet-1K validation set with off-the-shelf ResNet-50 classifier. %{\color{red} Extrapolate V1 curves to show gains.}
We provide results for 3 applicable connectors, 1) 2D average pooling of size 3$\times$3, 2) 2D depth-wise 3$\times$3 (27 parameters) and 3) 2D convolution 3$\times$3 (81 parameters) filters. To train the 2D-depth-wise conv and 2D-conv connectors, we used COCO-2017 validation set generated with rate-distortion optimized \textit{bmshj2018-hyperprior} codec at $q=8$ as ground truths. According to Eq.~\eqref{eq:V5}, we minimized the MSE (as $\mathcal{L}_D$) between the ground truths and the connector output images using an Adam optimizer at an initial learning rate of 0.1 reduced by a factor of 0.1 after each 10 epochs for 30 total epochs.

\begin{figure}[t]
	\centering
	\subfloat[ImageNet-1K]{\includegraphics[trim=10 10 40 20,clip,width=0.480\textwidth]{figures/imagenetacc1V5_3.pdf}}\hfill
	\subfloat[Cityscapes]{\includegraphics[trim=10 10 40 20,clip,width=0.480\textwidth]{figures/cityscapesV5_2.pdf}}
	\vspace{1mm}
	\caption{Inference results on the validation set with connectors. baseline: distortion optimized images, J-FT inference: images compressed and decompressed with codec optimized for detection (J-FT), J-FT Avgpool: J-FT images after average pooling, J-FT depthwise Conv: J-FT images after 2D depth-wise conv. connector, J-FT Conv: J-FT images after 2D conv. connector}\label{fig:imagenetCOCO}
\end{figure}

\begin{comment}
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/imagenetacc1V5_3.pdf}
\caption{Inference on ImageNet-1K. baseline: distortion optimized images, J-FT inference: images compressed and decompressed with codec optimized for detection (J-FT), J-FT Avgpool: J-FT images after average pooling, J-FT depthwise Conv: J-FT images after 2D depth-wise conv. connector, J-FT Conv: J-FT w/o C images after 2D conv. connector}\label{fig:imagenet}
\end{figure}
\end{comment}




Interestingly in Fig.~\ref{fig:imagenetCOCO}(a), the features optimized for COCO-detection achieve better classification accuracy compared to the images generated by rate-distortion optimized codecs on off-the-shelf ResNet trained with rate-distortion optimized images. Image classification being part of COCO-detection task can be a reason for this behavior. Note that the average pooling, depth wise convolution and convolution connectors achieve similar gains for ImageNet-1K inference which is significantly higher compared to the extrapolated inference on rate-distortion optimized images (baseline) at lower data rates.
\begin{comment}
\begin{figure}[t]
\centering
\includegraphics[width=1.0\linewidth]{figures/cityscapesV5_2.pdf}
\caption{Inference on Citysapes val set with Avgpool and 2d Conv connectors.}\label{fig:citiscapes}
\end{figure}
\end{comment}

As another secondary task, we tested the rate-accuracy performance of the images optimized for detection on Cityscapes data set for semantic segmentation. To obtain a segmentation model for inference, we trained a Deeplabv3+~\cite{chen2018encoder} with ResNet-50 backbone from scratch on the training set of the `left 8 bit' original images with fine annotations as the ground truths. Using the trained model, we repeated the similar inference steps on Cityscapes val set with the connectors trained with COCO val set. See Fig.~\ref{fig:imagenetCOCO}(b) for results.

Note that we used same pre-trained connectors for the inference on ImageNet-1K and Cityscapes. Even though the gains are similar for the connectors on ImageNet-1K classification, 2D convolution connector shows significant gains for the segmentation task on Cityscapes. Overall, application of a pre-trained connector enables the use of the images (optimized for a primary task) for inference at different secondary tasks even with better rate-accuracy performance.
\subsubsection{Fine-tuning the classifier for better performance}
Given that we have access to train/fine-tune the secondary task model, we observe that the latent/feature maps optimized for a primary task (detection) achieves significant accuracy gains for the secondary tasks from fine-tuning as well compared to fine-tuning on rate-distortion optimized images.
\begin{comment}
\begin{figure}[t]
\centering
\includegraphics[width=1.0\linewidth]{figures/imagenetacc1V6_2.pdf}
\caption{Fine-tuning the classifier on rate-detection optimized ImageNet-1K. baseline: inference  T-FT: fine-tuning on distortion optimized images. J-FT inference: inference on rate-detection optimized images J-FT T-FT: fine-tuning on rate-detection optimized images.}\label{fig:imagenet2}
\end{figure}
\end{comment}

\begin{figure}[t]
	\centering
	\subfloat[ImageNet-1K]{\includegraphics[trim=10 10 40 20,clip,width=0.480\textwidth]{figures/imagenetacc1V6_2.pdf}}\hfill
	\subfloat[Citysapes]{\includegraphics[trim=10 10 40 20,clip,width=0.480\textwidth]{figures/cityscapesV6_2.pdf}}
	\vspace{1mm}
	\caption{Fine-tuning the classifier on rate-detection optimized data sets. baseline: inference  T-FT: fine-tuning on distortion optimized images. J-FT inference: inference on rate-detection optimized images J-FT T-FT: fine-tuning on rate-detection optimized images.}\label{fig:imagenetCOCO2}
\end{figure}
To show the validity of this claim, we fine-tuned the off-the-shelf secondary task models with rate-detection accuracy optimized images separately at each BPP point (J-FT T-FT). As a baseline to compare with, we fine-tuned the secondary task models (T-FT) on images compressed with rate-distortion optimized \textit{bmshj2018-hyperprior}. Fig.~\ref{fig:imagenetCOCO2}(a)~ and ~\ref{fig:imagenetCOCO2}(b) compares the accuracy gains for ImageNet-1K and Cityscapes respectively.

For fine-tuning ResNet-50 classifier, we used an SGD optimizer to minimize the classification cross entropy at a learning rate of 0.001 and a momentum of 0.9 for 5 epochs for both \textit{bmshj2018-hyperprior} T-FT and J-FT T-FT settings. For Cityscapes segmentation, we used an SGD optimizer with a momentum of 0.9 and a weight decay of 5e-4 for 50 epochs at initial learning rate of 0.01 scheduled with a polynomial mode.

Note that the proposed method achieves 70\% top-1 classification accuracy at 0.21 BPP which is 55\% bandwidth saving compared to rate-distortion optimized \textit{bmshj2018-hyperprior} T-FT setting. Similarly the setting J-FT T-FT records 3\% classification accuracy improvement at 0.2 BPP compared to the baseline.
\begin{comment}
\begin{figure}[t]
\centering
\includegraphics[width=1.0\linewidth]{figures/cityscapesV6_2.pdf}
\caption{Fine-tuning the classifier on rate-detection optimized Cityscapes.}\label{fig:citiscapesV6}
\end{figure}
\end{comment}


==> 06_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
    This paper detailed what happens when a chain composed of a compression module and a task algorithm can be optimized end-to-end. The experiments show that it is possible to re-gain a lot in terms of accuracy at a given low-bitrate, when jointly fine-tuning the codec and the task or parts of them. However, the byproduct is that the decoded content from the fine-tuned codec becomes specialized to a specific task and a specific task algorithm. Connectors are then proposed to enable the use of the decoded content for secondary tasks, producing satisfactory results. The proposed system comes in handy when a primary task, performed remotely, requires an optimal trade-off between accuracy and bit-rate of the transmitted content, while the later needs to be used for secondary tasks or viewing by humans for instance. Experiments with object detection as primary task and image classification as secondary task validate the performance of the proposed approach, compared to directly using the codec.
    %{\color{red}Future work...}

